The Transit Light Curve Project. IV. Five Transits of the Exoplanet OGLE-TR-10b

We present I and B photometry of five distinct transits of the exoplanet OGLE-TR-10b. By modeling the light curves, we find the planetary radius to be R_P = 1.06 +/- 0.08 R_Jup and the stellar radius to be R_S = 1.10 +/- 0.07 R_sun. The uncertainties are dominated by statistical errors in the photometry. Our estimate of the planetary radius is smaller than previous estimates that were based on lower-precision photometry, and hence the planet is not as anomalously large as was previously thought. We provide updated determinations of all the system parameters, including the transit ephemerides.

==> tab1.tex <==
     IMACS & $I$ &   2453921.58279 &         1.00155 &         0.00248 \\
     IMACS & $I$ &   2453921.58608 &         1.00043 &         0.00186 \\
     IMACS & $I$ &   2453921.58785 &         1.00038 &         0.00188 \\
     IMACS & $I$ &   2453921.58855 &         1.00086 &         0.00201 \\
     IMACS & $I$ &   2453921.58926 &         0.99870 &         0.00186 \\
     IMACS & $I$ &   2453921.58998 &         1.00116 &         0.00186 \\
     IMACS & $I$ &   2453921.59067 &         1.00060 &         0.00193 \\
     IMACS & $I$ &   2453921.59137 &         1.00161 &         0.00189 \\
     IMACS & $I$ &   2453921.59207 &         0.99770 &         0.00189 \\
     IMACS & $I$ &   2453921.59277 &         0.99798 &         0.00194 \\
     IMACS & $I$ &   2453921.59348 &         0.99765 &         0.00189 \\
     IMACS & $I$ &   2453921.59418 &         0.99918 &         0.00194 \\
     IMACS & $I$ &   2453921.59583 &         1.00025 &         0.00198 \\
     IMACS & $I$ &   2453921.59653 &         1.00248 &         0.00201 \\
     IMACS & $I$ &   2453921.59723 &         0.99947 &         0.00192 \\
     IMACS & $I$ &   2453921.60113 &         1.00036 &         0.00185 \\
     IMACS & $I$ &   2453921.60183 &         0.99736 &         0.00189 \\
     IMACS & $I$ &   2453921.60253 &         1.00243 &         0.00190 \\
     IMACS & $I$ &   2453921.60324 &         0.99952 &         0.00197 \\
     IMACS & $I$ &   2453921.60394 &         0.99871 &         0.00196 \\
     IMACS & $I$ &   2453921.60463 &         0.99933 &         0.00192 \\
     IMACS & $I$ &   2453921.60532 &         1.00207 &         0.00193 \\
     IMACS & $I$ &   2453921.60603 &         1.00038 &         0.00190 \\
     IMACS & $I$ &   2453921.60674 &         0.99910 &         0.00202 \\
     IMACS & $I$ &   2453921.60743 &         1.00105 &         0.00186 \\
     IMACS & $I$ &   2453921.60825 &         0.99889 &         0.00192 \\
     IMACS & $I$ &   2453921.60897 &         1.00096 &         0.00186 \\
     IMACS & $I$ &   2453921.60966 &         1.00151 &         0.00194 \\
     IMACS & $I$ &   2453921.61038 &         1.00538 &         0.00201 \\
     IMACS & $I$ &   2453921.61128 &         1.00267 &         0.00189 \\
     IMACS & $I$ &   2453921.61214 &         1.00012 &         0.00186 \\
     IMACS & $I$ &   2453921.61290 &         0.99968 &         0.00192 \\
     IMACS & $I$ &   2453921.61378 &         0.99926 &         0.00186 \\
     IMACS & $I$ &   2453921.61459 &         0.99880 &         0.00180 \\
     IMACS & $I$ &   2453921.61537 &         1.00040 &         0.00200 \\
     IMACS & $I$ &   2453921.61608 &         0.99826 &         0.00201 \\
     IMACS & $I$ &   2453921.61677 &         1.00187 &         0.00193 \\
     IMACS & $I$ &   2453921.61747 &         1.00301 &         0.00188 \\
     IMACS & $I$ &   2453921.61816 &         1.00025 &         0.00188 \\
     IMACS & $I$ &   2453921.61887 &         0.99945 &         0.00188 \\
     IMACS & $I$ &   2453921.61956 &         1.00219 &         0.00193 \\
     IMACS & $I$ &   2453921.62027 &         0.99967 &         0.00193 \\
     IMACS & $I$ &   2453921.62096 &         1.00065 &         0.00188 \\
     IMACS & $I$ &   2453921.62165 &         1.00185 &         0.00190 \\
     IMACS & $I$ &   2453921.62235 &         0.99964 &         0.00192 \\
     IMACS & $I$ &   2453921.62310 &         1.00156 &         0.00193 \\
     IMACS & $I$ &   2453921.62379 &         1.00143 &         0.00189 \\
     IMACS & $I$ &   2453921.62449 &         0.99594 &         0.00182 \\
     IMACS & $I$ &   2453921.62520 &         0.99086 &         0.00192 \\
     IMACS & $I$ &   2453921.62589 &         0.99344 &         0.00186 \\
     IMACS & $I$ &   2453921.62659 &         0.99302 &         0.00190 \\
     IMACS & $I$ &   2453921.62728 &         0.99635 &         0.00181 \\
     IMACS & $I$ &   2453921.62868 &         0.99494 &         0.00197 \\
     IMACS & $I$ &   2453921.62937 &         0.99424 &         0.00206 \\
     IMACS & $I$ &   2453921.63077 &         0.99546 &         0.00189 \\
     IMACS & $I$ &   2453921.63147 &         0.99002 &         0.00196 \\
     IMACS & $I$ &   2453921.63217 &         0.99224 &         0.00192 \\
     IMACS & $I$ &   2453921.63287 &         0.98870 &         0.00200 \\
     IMACS & $I$ &   2453921.63356 &         0.98572 &         0.00190 \\
     IMACS & $I$ &   2453921.63426 &         0.98736 &         0.00193 \\
     IMACS & $I$ &   2453921.63496 &         0.99111 &         0.00194 \\
     IMACS & $I$ &   2453921.63566 &         0.99157 &         0.00182 \\
     IMACS & $I$ &   2453921.63635 &         0.99298 &         0.00188 \\
     IMACS & $I$ &   2453921.63714 &         0.99066 &         0.00182 \\
     IMACS & $I$ &   2453921.63785 &         0.98851 &         0.00186 \\
     IMACS & $I$ &   2453921.63854 &         0.99173 &         0.00193 \\
     IMACS & $I$ &   2453921.63924 &         0.99001 &         0.00184 \\
     IMACS & $I$ &   2453921.63993 &         0.99127 &         0.00188 \\
     IMACS & $I$ &   2453921.64064 &         0.98859 &         0.00182 \\
     IMACS & $I$ &   2453921.64133 &         0.99076 &         0.00189 \\
     IMACS & $I$ &   2453921.64202 &         0.98596 &         0.00184 \\
     IMACS & $I$ &   2453921.64273 &         0.99302 &         0.00189 \\
     IMACS & $I$ &   2453921.64342 &         0.99032 &         0.00180 \\
     IMACS & $I$ &   2453921.64413 &         0.98927 &         0.00189 \\
     IMACS & $I$ &   2453921.64482 &         0.99249 &         0.00188 \\
     IMACS & $I$ &   2453921.64553 &         0.98926 &         0.00182 \\
     IMACS & $I$ &   2453921.64622 &         0.99097 &         0.00182 \\
     IMACS & $I$ &   2453921.64692 &         0.99228 &         0.00189 \\
     IMACS & $I$ &   2453921.64763 &         0.98993 &         0.00186 \\
     IMACS & $I$ &   2453921.64832 &         0.99096 &         0.00182 \\
     IMACS & $I$ &   2453921.64902 &         0.98986 &         0.00180 \\
     IMACS & $I$ &   2453921.64971 &         0.99287 &         0.00190 \\
     IMACS & $I$ &   2453921.65042 &         0.98862 &         0.00188 \\
     IMACS & $I$ &   2453921.67528 &         0.98678 &         0.00200 \\
     IMACS & $I$ &   2453921.67763 &         0.98636 &         0.00201 \\
     IMACS & $I$ &   2453921.67845 &         0.98616 &         0.00194 \\
     IMACS & $I$ &   2453921.68412 &         0.98625 &         0.00189 \\
     IMACS & $I$ &   2453921.68482 &         0.99033 &         0.00202 \\
     IMACS & $I$ &   2453921.68558 &         0.98796 &         0.00198 \\
     IMACS & $I$ &   2453921.68629 &         0.98954 &         0.00204 \\
     IMACS & $I$ &   2453921.68702 &         0.98623 &         0.00204 \\
     IMACS & $I$ &   2453921.68773 &         0.98986 &         0.00202 \\
     IMACS & $I$ &   2453921.68843 &         0.98782 &         0.00204 \\
     IMACS & $I$ &   2453921.69612 &         0.98741 &         0.00198 \\
     IMACS & $I$ &   2453921.69693 &         0.98975 &         0.00193 \\
     IMACS & $I$ &   2453921.69764 &         0.98686 &         0.00194 \\
     IMACS & $I$ &   2453921.69833 &         0.99025 &         0.00204 \\
     IMACS & $I$ &   2453921.69904 &         0.98591 &         0.00201 \\
     IMACS & $I$ &   2453921.69973 &         0.98706 &         0.00202 \\
     IMACS & $I$ &   2453921.70044 &         0.98723 &         0.00196 \\
     IMACS & $I$ &   2453921.70113 &         0.99034 &         0.00194 \\
     IMACS & $I$ &   2453921.70184 &         0.99130 &         0.00197 \\
     IMACS & $I$ &   2453921.70253 &         0.99081 &         0.00201 \\
     IMACS & $I$ &   2453921.70750 &         0.99163 &         0.00209 \\
     IMACS & $I$ &   2453921.70823 &         0.99244 &         0.00193 \\
     IMACS & $I$ &   2453921.71114 &         0.98798 &         0.00201 \\
     IMACS & $I$ &   2453921.72695 &         0.99165 &         0.00185 \\
     IMACS & $I$ &   2453921.72842 &         0.98644 &         0.00190 \\
     IMACS & $I$ &   2453921.72915 &         0.98825 &         0.00185 \\
     IMACS & $I$ &   2453921.72986 &         0.99018 &         0.00197 \\
     IMACS & $I$ &   2453921.73059 &         0.98894 &         0.00196 \\
     IMACS & $I$ &   2453921.73132 &         0.98634 &         0.00198 \\
     IMACS & $I$ &   2453921.73204 &         0.99334 &         0.00201 \\
     IMACS & $I$ &   2453921.73277 &         0.99059 &         0.00201 \\
     IMACS & $I$ &   2453921.73347 &         0.99319 &         0.00198 \\
     IMACS & $I$ &   2453921.73416 &         0.98954 &         0.00196 \\
     IMACS & $I$ &   2453921.73557 &         0.99516 &         0.00186 \\
     IMACS & $I$ &   2453921.73627 &         0.99516 &         0.00189 \\
     IMACS & $I$ &   2453921.73698 &         0.99236 &         0.00192 \\
     IMACS & $I$ &   2453921.73767 &         0.99289 &         0.00204 \\
     IMACS & $I$ &   2453921.73838 &         0.99547 &         0.00192 \\
     IMACS & $I$ &   2453921.73908 &         0.99196 &         0.00185 \\
     IMACS & $I$ &   2453921.73978 &         0.99760 &         0.00190 \\
     IMACS & $I$ &   2453921.74055 &         0.99532 &         0.00188 \\
     IMACS & $I$ &   2453921.74126 &         0.99503 &         0.00206 \\
     IMACS & $I$ &   2453921.74195 &         0.99777 &         0.00193 \\
     IMACS & $I$ &   2453921.74336 &         1.00091 &         0.00184 \\
     IMACS & $I$ &   2453921.74408 &         0.99763 &         0.00189 \\
     IMACS & $I$ &   2453921.74478 &         0.99836 &         0.00194 \\
     IMACS & $I$ &   2453921.74548 &         1.00137 &         0.00198 \\
     IMACS & $I$ &   2453921.74619 &         0.99911 &         0.00197 \\
     IMACS & $I$ &   2453921.74689 &         0.99990 &         0.00197 \\
     IMACS & $I$ &   2453921.74760 &         1.00018 &         0.00186 \\
     IMACS & $I$ &   2453921.74831 &         1.00002 &         0.00192 \\
     IMACS & $I$ &   2453921.74900 &         1.00027 &         0.00186 \\
     IMACS & $I$ &   2453921.74971 &         0.99630 &         0.00198 \\
     IMACS & $I$ &   2453921.75041 &         0.99810 &         0.00204 \\
     IMACS & $I$ &   2453921.75112 &         1.00027 &         0.00185 \\
     IMACS & $I$ &   2453921.75183 &         0.99919 &         0.00194 \\
     IMACS & $I$ &   2453921.75252 &         0.99883 &         0.00193 \\
     IMACS & $I$ &   2453921.75323 &         1.00049 &         0.00188 \\
     IMACS & $I$ &   2453921.75392 &         1.00034 &         0.00190 \\
     IMACS & $I$ &   2453921.75463 &         1.00047 &         0.00185 \\
     IMACS & $I$ &   2453921.75532 &         0.99883 &         0.00188 \\
     IMACS & $I$ &   2453921.75603 &         0.99822 &         0.00186 \\
     IMACS & $I$ &   2453921.75673 &         1.00073 &         0.00193 \\
     IMACS & $I$ &   2453921.75744 &         1.00212 &         0.00184 \\
     IMACS & $I$ &   2453921.75816 &         1.00102 &         0.00192 \\
     IMACS & $I$ &   2453921.75888 &         1.00116 &         0.00186 \\
     IMACS & $I$ &   2453921.75961 &         0.99912 &         0.00189 \\
     IMACS & $I$ &   2453921.76034 &         1.00135 &         0.00181 \\
     IMACS & $I$ &   2453921.76107 &         1.00111 &         0.00190 \\
     IMACS & $I$ &   2453921.76178 &         1.00146 &         0.00189 \\
     IMACS & $I$ &   2453921.76247 &         1.00227 &         0.00182 \\
     IMACS & $I$ &   2453921.76317 &         1.00130 &         0.00186 \\
     IMACS & $I$ &   2453921.76387 &         1.00060 &         0.00185 \\
     IMACS & $I$ &   2453921.76457 &         0.99955 &         0.00194 \\
     IMACS & $I$ &   2453921.76526 &         0.99679 &         0.00188 \\
     IMACS & $I$ &   2453921.76597 &         1.00207 &         0.00182 \\
     IMACS & $I$ &   2453921.76667 &         0.99903 &         0.00182 \\
     IMACS & $I$ &   2453921.76740 &         1.00077 &         0.00189 \\
     IMACS & $I$ &   2453921.76814 &         0.99827 &         0.00185 \\
     IMACS & $I$ &   2453921.76917 &         1.00019 &         0.00188 \\
     IMACS & $I$ &   2453921.76989 &         0.99981 &         0.00190 \\
     IMACS & $I$ &   2453921.77062 &         1.00074 &         0.00194 \\
     IMACS & $I$ &   2453921.77135 &         1.00053 &         0.00189 \\
     IMACS & $I$ &   2453921.77207 &         1.00116 &         0.00190 \\
     IMACS & $I$ &   2453921.77567 &         0.99874 &         0.00192 \\
     IMACS & $I$ &   2453921.77785 &         0.99801 &         0.00188 \\
     IMACS & $I$ &   2453583.58158 &         0.99750 &         0.00120 \\
     IMACS & $I$ &   2453583.58224 &         0.99889 &         0.00127 \\
     IMACS & $I$ &   2453583.58299 &         0.99753 &         0.00123 \\
     IMACS & $I$ &   2453583.58375 &         0.99725 &         0.00120 \\
     IMACS & $I$ &   2453583.58439 &         1.00026 &         0.00118 \\
     IMACS & $I$ &   2453583.58502 &         0.99729 &         0.00117 \\
     IMACS & $I$ &   2453583.58567 &         0.99796 &         0.00118 \\
     IMACS & $I$ &   2453583.58632 &         0.99645 &         0.00120 \\
     IMACS & $I$ &   2453583.58699 &         0.99792 &         0.00120 \\
     IMACS & $I$ &   2453583.58964 &         0.99682 &         0.00123 \\
     IMACS & $I$ &   2453583.59030 &         0.99578 &         0.00125 \\
     IMACS & $I$ &   2453583.59094 &         0.99525 &         0.00123 \\
     IMACS & $I$ &   2453583.59157 &         0.99287 &         0.00123 \\
     IMACS & $I$ &   2453583.59222 &         0.99303 &         0.00122 \\
     IMACS & $I$ &   2453583.59290 &         0.99368 &         0.00123 \\
     IMACS & $I$ &   2453583.59354 &         0.99207 &         0.00122 \\
     IMACS & $I$ &   2453583.59418 &         0.99294 &         0.00120 \\
     IMACS & $I$ &   2453583.59483 &         0.99325 &         0.00118 \\
     IMACS & $I$ &   2453583.59546 &         0.99223 &         0.00130 \\
     IMACS & $I$ &   2453583.59620 &         0.99156 &         0.00120 \\
     IMACS & $I$ &   2453583.59684 &         0.99061 &         0.00123 \\
     IMACS & $I$ &   2453583.59748 &         0.99061 &         0.00123 \\
     IMACS & $I$ &   2453583.59813 &         0.98982 &         0.00125 \\
     IMACS & $I$ &   2453583.59877 &         0.99076 &         0.00123 \\
     IMACS & $I$ &   2453583.59942 &         0.99055 &         0.00122 \\
     IMACS & $I$ &   2453583.60006 &         0.98962 &         0.00120 \\
     IMACS & $I$ &   2453583.60069 &         0.98647 &         0.00131 \\
     IMACS & $I$ &   2453583.60134 &         0.98946 &         0.00127 \\
     IMACS & $I$ &   2453583.60199 &         0.98917 &         0.00122 \\
     IMACS & $I$ &   2453583.60270 &         0.98767 &         0.00128 \\
     IMACS & $I$ &   2453583.60333 &         0.98913 &         0.00125 \\
     IMACS & $I$ &   2453583.60397 &         0.98840 &         0.00123 \\
     IMACS & $I$ &   2453583.60461 &         0.98969 &         0.00122 \\
     IMACS & $I$ &   2453583.60524 &         0.99044 &         0.00123 \\
     IMACS & $I$ &   2453583.60588 &         0.98942 &         0.00122 \\
     IMACS & $I$ &   2453583.60653 &         0.98838 &         0.00125 \\
     IMACS & $I$ &   2453583.60716 &         0.99046 &         0.00123 \\
     IMACS & $I$ &   2453583.60780 &         0.99082 &         0.00122 \\
     IMACS & $I$ &   2453583.60845 &         0.99060 &         0.00123 \\
     IMACS & $I$ &   2453583.60909 &         0.98947 &         0.00122 \\
     IMACS & $I$ &   2453583.60972 &         0.98979 &         0.00122 \\
     IMACS & $I$ &   2453583.61036 &         0.98955 &         0.00122 \\
     IMACS & $I$ &   2453583.61099 &         0.99030 &         0.00127 \\
     IMACS & $I$ &   2453583.61163 &         0.99008 &         0.00125 \\
     IMACS & $I$ &   2453583.61227 &         0.98821 &         0.00131 \\
     IMACS & $I$ &   2453583.61290 &         0.98975 &         0.00122 \\
     IMACS & $I$ &   2453583.61354 &         0.98999 &         0.00127 \\
     IMACS & $I$ &   2453583.61418 &         0.98902 &         0.00123 \\
     IMACS & $I$ &   2453583.61483 &         0.98842 &         0.00125 \\
     IMACS & $I$ &   2453583.61547 &         0.98732 &         0.00120 \\
     IMACS & $I$ &   2453583.61611 &         0.99036 &         0.00120 \\
     IMACS & $I$ &   2453583.61675 &         0.98620 &         0.00123 \\
     IMACS & $I$ &   2453583.61738 &         0.99056 &         0.00123 \\
     IMACS & $I$ &   2453583.61802 &         0.98928 &         0.00123 \\
     IMACS & $I$ &   2453583.61866 &         0.98908 &         0.00123 \\
     IMACS & $I$ &   2453583.61929 &         0.98844 &         0.00122 \\
     IMACS & $I$ &   2453583.61994 &         0.99016 &         0.00123 \\
     IMACS & $I$ &   2453583.62058 &         0.98922 &         0.00122 \\
     IMACS & $I$ &   2453583.62121 &         0.99021 &         0.00123 \\
     IMACS & $I$ &   2453583.62186 &         0.98842 &         0.00122 \\
     IMACS & $I$ &   2453583.62251 &         0.98821 &         0.00123 \\
     IMACS & $I$ &   2453583.62316 &         0.99105 &         0.00123 \\
     IMACS & $I$ &   2453583.62379 &         0.98830 &         0.00122 \\
     IMACS & $I$ &   2453583.62443 &         0.99019 &         0.00122 \\
     IMACS & $I$ &   2453583.62507 &         0.98888 &         0.00122 \\
     IMACS & $I$ &   2453583.62570 &         0.98937 &         0.00120 \\
     IMACS & $I$ &   2453583.62634 &         0.98944 &         0.00122 \\
     IMACS & $I$ &   2453583.62698 &         0.98906 &         0.00122 \\
     IMACS & $I$ &   2453583.62761 &         0.98807 &         0.00122 \\
     IMACS & $I$ &   2453583.62826 &         0.99088 &         0.00122 \\
     IMACS & $I$ &   2453583.62890 &         0.98970 &         0.00120 \\
     IMACS & $I$ &   2453583.62953 &         0.99047 &         0.00118 \\
     IMACS & $I$ &   2453583.63017 &         0.98868 &         0.00120 \\
     IMACS & $I$ &   2453583.63082 &         0.98949 &         0.00118 \\
     IMACS & $I$ &   2453583.63146 &         0.98891 &         0.00120 \\
     IMACS & $I$ &   2453583.63209 &         0.98913 &         0.00118 \\
     IMACS & $I$ &   2453583.63273 &         0.98957 &         0.00118 \\
     IMACS & $I$ &   2453583.63337 &         0.98938 &         0.00118 \\
     IMACS & $I$ &   2453583.63400 &         0.99042 &         0.00120 \\
     IMACS & $I$ &   2453583.63464 &         0.98996 &         0.00118 \\
     IMACS & $I$ &   2453583.63529 &         0.98959 &         0.00118 \\
     IMACS & $I$ &   2453583.63592 &         0.98932 &         0.00120 \\
     IMACS & $I$ &   2453583.63656 &         0.98957 &         0.00118 \\
     IMACS & $I$ &   2453583.63721 &         0.99008 &         0.00118 \\
     IMACS & $I$ &   2453583.63784 &         0.98962 &         0.00118 \\
     IMACS & $I$ &   2453583.63848 &         0.98942 &         0.00118 \\
     IMACS & $I$ &   2453583.63912 &         0.98924 &         0.00118 \\
     IMACS & $I$ &   2453583.63975 &         0.99244 &         0.00118 \\
     IMACS & $I$ &   2453583.64039 &         0.98950 &         0.00115 \\
     IMACS & $I$ &   2453583.64104 &         0.98959 &         0.00117 \\
     IMACS & $I$ &   2453583.64168 &         0.98911 &         0.00122 \\
     IMACS & $I$ &   2453583.64231 &         0.98862 &         0.00122 \\
     IMACS & $I$ &   2453583.64295 &         0.98872 &         0.00122 \\
     IMACS & $I$ &   2453583.64359 &         0.98950 &         0.00122 \\
     IMACS & $I$ &   2453583.64422 &         0.98852 &         0.00122 \\
     IMACS & $I$ &   2453583.64486 &         0.98881 &         0.00122 \\
     IMACS & $I$ &   2453583.64549 &         0.99055 &         0.00122 \\
     IMACS & $I$ &   2453583.64613 &         0.99061 &         0.00120 \\
     IMACS & $I$ &   2453583.64677 &         0.99113 &         0.00118 \\
     IMACS & $I$ &   2453583.64742 &         0.98836 &         0.00120 \\
     IMACS & $I$ &   2453583.64805 &         0.98897 &         0.00120 \\
     IMACS & $I$ &   2453583.64869 &         0.98991 &         0.00122 \\
     IMACS & $I$ &   2453583.64933 &         0.98986 &         0.00122 \\
     IMACS & $I$ &   2453583.64996 &         0.99048 &         0.00123 \\
     IMACS & $I$ &   2453583.65060 &         0.98900 &         0.00123 \\
     IMACS & $I$ &   2453583.65124 &         0.98900 &         0.00123 \\
     IMACS & $I$ &   2453583.65187 &         0.98935 &         0.00123 \\
     IMACS & $I$ &   2453583.65251 &         0.98721 &         0.00125 \\
     IMACS & $I$ &   2453583.65314 &         0.98893 &         0.00125 \\
     IMACS & $I$ &   2453583.65378 &         0.98783 &         0.00125 \\
     IMACS & $I$ &   2453583.65442 &         0.98756 &         0.00125 \\
     IMACS & $I$ &   2453583.65505 &         0.99013 &         0.00122 \\
     IMACS & $I$ &   2453583.65569 &         0.98953 &         0.00120 \\
     IMACS & $I$ &   2453583.65634 &         0.98816 &         0.00122 \\
     IMACS & $I$ &   2453583.65698 &         0.98822 &         0.00122 \\
     IMACS & $I$ &   2453583.65762 &         0.98952 &         0.00120 \\
     IMACS & $I$ &   2453583.65827 &         0.98884 &         0.00120 \\
     IMACS & $I$ &   2453583.65891 &         0.98941 &         0.00122 \\
     IMACS & $I$ &   2453583.65954 &         0.98780 &         0.00122 \\
     IMACS & $I$ &   2453583.66023 &         0.98867 &         0.00120 \\
     IMACS & $I$ &   2453583.66086 &         0.98867 &         0.00123 \\
     IMACS & $I$ &   2453583.66150 &         0.98835 &         0.00120 \\
     IMACS & $I$ &   2453583.66214 &         0.98938 &         0.00122 \\
     IMACS & $I$ &   2453583.66277 &         0.98988 &         0.00122 \\
     IMACS & $I$ &   2453583.66341 &         0.98849 &         0.00122 \\
     IMACS & $I$ &   2453583.66405 &         0.98841 &         0.00122 \\
     IMACS & $I$ &   2453583.66468 &         0.98949 &         0.00120 \\
     IMACS & $I$ &   2453583.66532 &         0.98823 &         0.00122 \\
     IMACS & $I$ &   2453583.66596 &         0.98746 &         0.00122 \\
     IMACS & $I$ &   2453583.66660 &         0.98847 &         0.00122 \\
     IMACS & $I$ &   2453583.66724 &         0.98776 &         0.00122 \\
     IMACS & $I$ &   2453583.66788 &         0.98975 &         0.00123 \\
     IMACS & $I$ &   2453583.66851 &         0.98860 &         0.00123 \\
     IMACS & $I$ &   2453583.66915 &         0.98929 &         0.00120 \\
     IMACS & $I$ &   2453583.66979 &         0.98822 &         0.00122 \\
     IMACS & $I$ &   2453583.67042 &         0.98835 &         0.00122 \\
     IMACS & $I$ &   2453583.67106 &         0.98917 &         0.00122 \\
     IMACS & $I$ &   2453583.67170 &         0.98977 &         0.00122 \\
     IMACS & $I$ &   2453583.67233 &         0.98878 &         0.00122 \\
     IMACS & $I$ &   2453583.67297 &         0.98748 &         0.00122 \\
     IMACS & $I$ &   2453583.67361 &         0.98947 &         0.00120 \\
     IMACS & $I$ &   2453583.67424 &         0.98900 &         0.00122 \\
     IMACS & $I$ &   2453583.67488 &         0.98917 &         0.00122 \\
     IMACS & $I$ &   2453583.67552 &         0.99015 &         0.00122 \\
     IMACS & $I$ &   2453583.67615 &         0.98806 &         0.00122 \\
     IMACS & $I$ &   2453583.67679 &         0.98990 &         0.00122 \\
     IMACS & $I$ &   2453583.67742 &         0.98890 &         0.00122 \\
     IMACS & $I$ &   2453583.67806 &         0.99044 &         0.00120 \\
     IMACS & $I$ &   2453583.67870 &         0.99000 &         0.00120 \\
     IMACS & $I$ &   2453583.67960 &         0.98974 &         0.00120 \\
     IMACS & $I$ &   2453583.68024 &         0.98947 &         0.00120 \\
     IMACS & $I$ &   2453583.68087 &         0.98772 &         0.00120 \\
     IMACS & $I$ &   2453583.68151 &         0.99023 &         0.00120 \\
     IMACS & $I$ &   2453583.68215 &         0.98954 &         0.00122 \\
     IMACS & $I$ &   2453583.68278 &         0.98966 &         0.00122 \\
     IMACS & $I$ &   2453583.68342 &         0.99053 &         0.00120 \\
     IMACS & $I$ &   2453583.68406 &         0.98868 &         0.00122 \\
     IMACS & $I$ &   2453583.68469 &         0.98898 &         0.00122 \\
     IMACS & $I$ &   2453583.68533 &         0.98991 &         0.00120 \\
     IMACS & $I$ &   2453583.68597 &         0.98794 &         0.00120 \\
     IMACS & $I$ &   2453583.68660 &         0.99051 &         0.00118 \\
     IMACS & $I$ &   2453583.68724 &         0.99140 &         0.00117 \\
     IMACS & $I$ &   2453583.68788 &         0.99096 &         0.00117 \\
     IMACS & $I$ &   2453583.68851 &         0.98914 &         0.00117 \\
     IMACS & $I$ &   2453583.68915 &         0.99184 &         0.00117 \\
     IMACS & $I$ &   2453583.68979 &         0.99007 &         0.00115 \\
     IMACS & $I$ &   2453583.69042 &         0.99023 &         0.00115 \\
     IMACS & $I$ &   2453583.69106 &         0.99019 &         0.00117 \\
     IMACS & $I$ &   2453583.69170 &         0.99264 &         0.00115 \\
     IMACS & $I$ &   2453583.69233 &         0.99066 &         0.00117 \\
     IMACS & $I$ &   2453583.69297 &         0.99057 &         0.00120 \\
     IMACS & $I$ &   2453583.69361 &         0.98931 &         0.00117 \\
     IMACS & $I$ &   2453583.69425 &         0.99017 &         0.00118 \\
     IMACS & $I$ &   2453583.69489 &         0.99048 &         0.00118 \\
     IMACS & $I$ &   2453583.69553 &         0.98983 &         0.00118 \\
     IMACS & $I$ &   2453583.69616 &         0.99077 &         0.00118 \\
     IMACS & $I$ &   2453583.69680 &         0.99215 &         0.00120 \\
     IMACS & $I$ &   2453583.69744 &         0.99092 &         0.00125 \\
     IMACS & $I$ &   2453583.69807 &         0.98963 &         0.00127 \\
     IMACS & $I$ &   2453583.69874 &         0.99329 &         0.00125 \\
     IMACS & $I$ &   2453583.69938 &         0.99357 &         0.00125 \\
     IMACS & $I$ &   2453583.70002 &         0.99269 &         0.00127 \\
     IMACS & $I$ &   2453583.70065 &         0.99290 &         0.00127 \\
     IMACS & $I$ &   2453583.70129 &         0.99422 &         0.00125 \\
     IMACS & $I$ &   2453583.70193 &         0.99501 &         0.00120 \\
     IMACS & $I$ &   2453583.70256 &         0.99564 &         0.00117 \\
     IMACS & $I$ &   2453583.70320 &         0.99665 &         0.00117 \\
     IMACS & $I$ &   2453583.70384 &         0.99887 &         0.00115 \\
     IMACS & $I$ &   2453583.70447 &         0.99796 &         0.00113 \\
     IMACS & $I$ &   2453583.70511 &         1.00149 &         0.00117 \\
     IMACS & $I$ &   2453583.70574 &         0.99634 &         0.00118 \\
     IMACS & $I$ &   2453583.70638 &         1.00042 &         0.00117 \\
     IMACS & $I$ &   2453583.70702 &         0.99890 &         0.00117 \\
     IMACS & $I$ &   2453583.70766 &         0.99735 &         0.00117 \\
     IMACS & $I$ &   2453583.70829 &         0.99656 &         0.00118 \\
     IMACS & $I$ &   2453583.70893 &         1.00235 &         0.00118 \\
     IMACS & $I$ &   2453583.70956 &         0.99970 &         0.00115 \\
     IMACS & $I$ &   2453583.71020 &         1.00009 &         0.00113 \\
     IMACS & $I$ &   2453583.71084 &         0.99931 &         0.00115 \\
     IMACS & $I$ &   2453583.71147 &         1.00126 &         0.00115 \\
     IMACS & $I$ &   2453583.71211 &         1.00030 &         0.00113 \\
     IMACS & $I$ &   2453583.71275 &         1.00122 &         0.00115 \\
     IMACS & $I$ &   2453583.71338 &         1.00141 &         0.00113 \\
     IMACS & $I$ &   2453583.71402 &         1.00163 &         0.00115 \\
     IMACS & $I$ &   2453583.71466 &         1.00078 &         0.00112 \\
     IMACS & $I$ &   2453583.71529 &         1.00157 &         0.00113 \\
     IMACS & $I$ &   2453583.71593 &         0.99773 &         0.00117 \\
     IMACS & $I$ &   2453583.71657 &         0.99811 &         0.00118 \\
     IMACS & $I$ &   2453583.71720 &         0.99859 &         0.00117 \\
     IMACS & $I$ &   2453583.71899 &         0.99957 &         0.00115 \\
     IMACS & $I$ &   2453583.71962 &         0.99896 &         0.00117 \\
     IMACS & $I$ &   2453583.72170 &         1.00285 &         0.00111 \\
     IMACS & $I$ &   2453583.72346 &         0.99947 &         0.00115 \\
     IMACS & $I$ &   2453583.72536 &         0.99823 &         0.00120 \\
     IMACS & $I$ &   2453583.72717 &         1.00311 &         0.00118 \\
     IMACS & $I$ &   2453583.72800 &         0.99941 &         0.00117 \\
     IMACS & $I$ &   2453583.72864 &         1.00036 &         0.00117 \\
     IMACS & $I$ &   2453583.72927 &         0.99717 &         0.00117 \\
     IMACS & $I$ &   2453583.72991 &         1.00042 &         0.00117 \\
     MagIC & $I$ &   2452851.68436 &         1.00108 &         0.00089 \\
     MagIC & $I$ &   2452851.68657 &         0.99943 &         0.00091 \\
     MagIC & $I$ &   2452851.68874 &         0.99464 &         0.00093 \\
     MagIC & $I$ &   2452851.69092 &         0.99359 &         0.00087 \\
     MagIC & $I$ &   2452851.69310 &         0.99096 &         0.00096 \\
     MagIC & $I$ &   2452851.69527 &         0.99002 &         0.00093 \\
     MagIC & $I$ &   2452851.69761 &         0.99047 &         0.00089 \\
     MagIC & $I$ &   2452851.69979 &         0.99094 &         0.00091 \\
     MagIC & $I$ &   2452851.70196 &         0.99039 &         0.00091 \\
     MagIC & $I$ &   2452851.70415 &         0.99067 &         0.00089 \\
     MagIC & $I$ &   2452851.70633 &         0.98925 &         0.00091 \\
     MagIC & $I$ &   2452851.70857 &         0.99008 &         0.00087 \\
     MagIC & $I$ &   2452851.71075 &         0.98962 &         0.00087 \\
     MagIC & $I$ &   2452851.71292 &         0.99009 &         0.00089 \\
     MagIC & $I$ &   2452851.71510 &         0.98955 &         0.00091 \\
     MagIC & $I$ &   2452851.71727 &         0.99007 &         0.00091 \\
     MagIC & $I$ &   2452851.71945 &         0.98925 &         0.00093 \\
     MagIC & $I$ &   2452851.72162 &         0.98855 &         0.00093 \\
     MagIC & $I$ &   2452851.72380 &         0.98899 &         0.00089 \\
     MagIC & $I$ &   2452851.72598 &         0.98873 &         0.00089 \\
     MagIC & $I$ &   2452851.72815 &         0.98899 &         0.00079 \\
     MagIC & $I$ &   2452851.73042 &         0.98884 &         0.00093 \\
     MagIC & $I$ &   2452851.73260 &         0.98732 &         0.00091 \\
     MagIC & $I$ &   2452851.73477 &         0.98762 &         0.00102 \\
     MagIC & $I$ &   2452851.73695 &         0.98879 &         0.00098 \\
     MagIC & $I$ &   2452851.73912 &         0.98964 &         0.00091 \\
     MagIC & $I$ &   2452851.74130 &         0.98944 &         0.00093 \\
     MagIC & $I$ &   2452851.74347 &         0.98972 &         0.00091 \\
     MagIC & $I$ &   2452848.69226 &         0.99128 &         0.00052 \\
     MagIC & $I$ &   2452848.69445 &         0.99150 &         0.00052 \\
     MagIC & $I$ &   2452848.69662 &         0.99337 &         0.00054 \\
     MagIC & $I$ &   2452848.69880 &         0.99554 &         0.00053 \\
     MagIC & $I$ &   2452848.70103 &         0.99754 &         0.00054 \\
     MagIC & $I$ &   2452848.70321 &         0.99918 &         0.00054 \\
     MagIC & $I$ &   2452848.70540 &         1.00073 &         0.00054 \\
     MagIC & $I$ &   2452848.70757 &         0.99989 &         0.00055 \\
     MagIC & $I$ &   2452848.70974 &         1.00020 &         0.00055 \\
     MagIC & $I$ &   2452848.71844 &         0.99898 &         0.00055 \\
     MagIC & $I$ &   2452848.72061 &         0.99965 &         0.00054 \\
     MagIC & $I$ &   2452848.72280 &         0.99967 &         0.00055 \\
     MagIC & $I$ &   2452848.72497 &         0.99966 &         0.00055 \\
     MagIC & $I$ &   2452848.72715 &         1.00049 &         0.00055 \\
     MagIC & $I$ &   2452848.72933 &         0.99998 &         0.00053 \\
     MagIC & $I$ &   2452848.73151 &         1.00106 &         0.00052 \\
     MagIC & $I$ &   2452848.73367 &         0.99951 &         0.00053 \\
     MagIC & $I$ &   2452848.73586 &         0.99974 &         0.00054 \\
     MagIC & $I$ &   2452848.73803 &         1.00035 &         0.00054 \\
     MagIC & $I$ &   2452848.74022 &         1.00099 &         0.00054 \\
     MagIC & $I$ &   2452848.74240 &         0.99969 &         0.00055 \\
     MagIC & $I$ &   2452848.74457 &         0.99972 &         0.00054 \\
     MagIC & $I$ &   2452848.74892 &         0.99961 &         0.00055 \\
     MagIC & $I$ &   2452761.77735 &         0.98993 &         0.00129 \\
     MagIC & $I$ &   2452761.77968 &         0.98983 &         0.00132 \\
     MagIC & $I$ &   2452761.78225 &         0.99052 &         0.00129 \\
     MagIC & $I$ &   2452761.78454 &         0.98983 &         0.00132 \\
     MagIC & $I$ &   2452761.78677 &         0.98971 &         0.00129 \\
     MagIC & $I$ &   2452761.78885 &         0.98876 &         0.00092 \\
     MagIC & $I$ &   2452761.79086 &         0.98945 &         0.00092 \\
     MagIC & $I$ &   2452761.79274 &         0.98917 &         0.00092 \\
     MagIC & $I$ &   2452761.79459 &         0.98854 &         0.00092 \\
     MagIC & $I$ &   2452761.79644 &         0.98856 &         0.00094 \\
     MagIC & $I$ &   2452761.79828 &         0.98806 &         0.00092 \\
     MagIC & $I$ &   2452761.80015 &         0.98782 &         0.00092 \\
     MagIC & $I$ &   2452761.80211 &         0.98775 &         0.00092 \\
     MagIC & $I$ &   2452761.81182 &         0.98753 &         0.00094 \\
     MagIC & $I$ &   2452761.81393 &         0.98764 &         0.00092 \\
     MagIC & $I$ &   2452761.81579 &         0.98713 &         0.00092 \\
     MagIC & $I$ &   2452761.81644 &         0.98587 &         0.00094 \\
     MagIC & $I$ &   2452761.83843 &         0.99084 &         0.00094 \\
     MagIC & $I$ &   2452761.84032 &         0.99040 &         0.00089 \\
     MagIC & $I$ &   2452761.84247 &         0.98948 &         0.00092 \\
     MagIC & $I$ &   2452761.84451 &         0.98889 &         0.00094 \\
     MagIC & $I$ &   2452761.84842 &         0.99188 &         0.00139 \\
     MagIC & $I$ &   2452761.85674 &         0.99605 &         0.00137 \\
     MagIC & $I$ &   2452761.85883 &         0.99608 &         0.00119 \\
     MagIC & $I$ &   2452761.86093 &         0.99512 &         0.00137 \\
     MagIC & $I$ &   2452761.86312 &         0.99626 &         0.00134 \\
     MagIC & $I$ &   2452761.86513 &         0.99804 &         0.00092 \\
     MagIC & $I$ &   2452761.86704 &         0.99940 &         0.00119 \\
     MagIC & $I$ &   2452761.86918 &         1.00023 &         0.00142 \\
     MagIC & $I$ &   2452761.87141 &         1.00070 &         0.00137 \\
     MagIC & $I$ &   2452761.87360 &         1.00126 &         0.00139 \\
     MagIC & $I$ &   2452761.87577 &         1.00034 &         0.00137 \\
     MagIC & $I$ &   2452761.87795 &         1.00021 &         0.00142 \\
     MagIC & $I$ &   2452761.88013 &         1.00122 &         0.00137 \\
     MagIC & $I$ &   2452761.88231 &         1.00212 &         0.00137 \\
     MagIC & $I$ &   2452761.88449 &         1.00095 &         0.00137 \\
     MagIC & $I$ &   2452761.88667 &         1.00036 &         0.00137 \\
     MagIC & $I$ &   2452761.88896 &         1.00091 &         0.00132 \\
     MagIC & $I$ &   2452761.89130 &         1.00049 &         0.00137 \\
     MagIC & $I$ &   2452761.89347 &         1.00020 &         0.00134 \\
     MagIC & $I$ &   2452761.89565 &         0.99997 &         0.00134 \\
     MagIC & $I$ &   2452761.89788 &         1.00047 &         0.00134 \\
     MagIC & $I$ &   2452761.90021 &         1.00130 &         0.00142 \\
     MagIC & $I$ &   2452761.90239 &         1.00068 &         0.00134 \\
     MagIC & $I$ &   2452761.90456 &         1.00148 &         0.00137 \\
     MagIC & $I$ &   2452761.90674 &         1.00069 &         0.00137 \\
     MagIC & $I$ &   2452761.90891 &         1.00075 &         0.00132 \\
     MagIC & $I$ &   2452761.91109 &         1.00058 &         0.00139 \\
     MagIC & $I$ &   2452761.91327 &         1.00043 &         0.00139 \\
     MagIC & $I$ &   2452761.91467 &         1.00003 &         0.00127 \\
     MagIC & $I$ &   2452761.91720 &         1.00006 &         0.00107 \\
     MagIC & $I$ &   2452761.91944 &         0.99887 &         0.00117 \\
     MagIC & $I$ &   2452761.92162 &         0.99894 &         0.00109 \\
     MagIC & $I$ &   2452761.92380 &         0.99991 &         0.00127 \\
     MagIC & $I$ &   2452761.92603 &         0.99969 &         0.00139 \\
     MagIC & $I$ &   2452761.92821 &         0.99804 &         0.00137 \\
     MagIC & $I$ &   2452761.93085 &         1.00007 &         0.00127 \\
     MagIC & $I$ &   2452761.93308 &         0.99895 &         0.00144 \\
     MagIC & $B$ &   2452851.68325 &         1.00446 &         0.00190 \\
     MagIC & $B$ &   2452851.68548 &         0.99936 &         0.00190 \\
     MagIC & $B$ &   2452851.68766 &         0.99699 &         0.00186 \\
     MagIC & $B$ &   2452851.68983 &         0.99727 &         0.00174 \\
     MagIC & $B$ &   2452851.69201 &         0.99290 &         0.00177 \\
     MagIC & $B$ &   2452851.69418 &         0.99291 &         0.00192 \\
     MagIC & $B$ &   2452851.69652 &         0.99060 &         0.00189 \\
     MagIC & $B$ &   2452851.69870 &         0.99114 &         0.00183 \\
     MagIC & $B$ &   2452851.70087 &         0.99138 &         0.00183 \\
     MagIC & $B$ &   2452851.70306 &         0.99050 &         0.00187 \\
     MagIC & $B$ &   2452851.70524 &         0.98750 &         0.00190 \\
     MagIC & $B$ &   2452851.70748 &         0.98985 &         0.00157 \\
     MagIC & $B$ &   2452851.70966 &         0.98821 &         0.00177 \\
     MagIC & $B$ &   2452851.71183 &         0.98740 &         0.00174 \\
     MagIC & $B$ &   2452851.71401 &         0.99224 &         0.00155 \\
     MagIC & $B$ &   2452851.71618 &         0.98838 &         0.00187 \\
     MagIC & $B$ &   2452851.71836 &         0.98716 &         0.00183 \\
     MagIC & $B$ &   2452851.72054 &         0.98733 &         0.00184 \\
     MagIC & $B$ &   2452851.72271 &         0.98690 &         0.00183 \\
     MagIC & $B$ &   2452851.72489 &         0.98641 &         0.00180 \\
     MagIC & $B$ &   2452851.72706 &         0.98964 &         0.00174 \\
     MagIC & $B$ &   2452851.72933 &         0.98862 &         0.00180 \\
     MagIC & $B$ &   2452851.73151 &         0.98518 &         0.00184 \\
     MagIC & $B$ &   2452851.73368 &         0.98602 &         0.00183 \\
     MagIC & $B$ &   2452851.73586 &         0.98652 &         0.00195 \\
     MagIC & $B$ &   2452851.73804 &         0.98768 &         0.00187 \\
     MagIC & $B$ &   2452851.74021 &         0.98845 &         0.00187 \\
     MagIC & $B$ &   2452851.74239 &         0.98825 &         0.00187 \\
     MagIC & $B$ &   2452851.74456 &         0.99082 &         0.00183 \\
     MagIC & $B$ &   2452848.69118 &         0.98896 &         0.00185 \\
     MagIC & $B$ &   2452848.69335 &         0.99507 &         0.00176 \\
     MagIC & $B$ &   2452848.69553 &         0.99088 &         0.00184 \\
     MagIC & $B$ &   2452848.69771 &         0.99638 &         0.00188 \\
     MagIC & $B$ &   2452848.69989 &         0.99762 &         0.00188 \\
     MagIC & $B$ &   2452848.70213 &         0.99784 &         0.00188 \\
     MagIC & $B$ &   2452848.70431 &         0.99939 &         0.00194 \\
     MagIC & $B$ &   2452848.70648 &         1.00162 &         0.00194 \\
     MagIC & $B$ &   2452848.70866 &         0.99935 &         0.00191 \\
     MagIC & $B$ &   2452848.71082 &         0.99947 &         0.00203 \\
     MagIC & $B$ &   2452848.71300 &         1.00113 &         0.00206 \\
     MagIC & $B$ &   2452848.71518 &         1.00340 &         0.00203 \\
     MagIC & $B$ &   2452848.71735 &         1.00153 &         0.00191 \\
     MagIC & $B$ &   2452848.71953 &         1.00165 &         0.00185 \\
     MagIC & $B$ &   2452848.72171 &         1.00076 &         0.00191 \\
     MagIC & $B$ &   2452848.72389 &         0.99914 &         0.00190 \\
     MagIC & $B$ &   2452848.72607 &         0.99645 &         0.00187 \\
     MagIC & $B$ &   2452848.73042 &         0.99938 &         0.00176 \\
     MagIC & $B$ &   2452848.73258 &         0.99983 &         0.00182 \\
     MagIC & $B$ &   2452848.73476 &         1.00022 &         0.00184 \\
     MagIC & $B$ &   2452761.77626 &         0.99062 &         0.00245 \\
     MagIC & $B$ &   2452761.77845 &         0.98930 &         0.00245 \\
     MagIC & $B$ &   2452761.78080 &         0.98815 &         0.00245 \\
     MagIC & $B$ &   2452761.78344 &         0.98846 &         0.00245 \\
     MagIC & $B$ &   2452761.78567 &         0.98751 &         0.00245 \\
     MagIC & $B$ &   2452761.78787 &         0.98993 &         0.00243 \\
     MagIC & $B$ &   2452761.78980 &         0.98934 &         0.00245 \\
     MagIC & $B$ &   2452761.79183 &         0.98999 &         0.00245 \\
     MagIC & $B$ &   2452761.79366 &         0.98999 &         0.00245 \\
     MagIC & $B$ &   2452761.79551 &         0.99091 &         0.00247 \\
     MagIC & $B$ &   2452761.79737 &         0.99117 &         0.00245 \\
     MagIC & $B$ &   2452761.79921 &         0.98933 &         0.00245 \\
     MagIC & $B$ &   2452761.80109 &         0.98852 &         0.00245 \\
     MagIC & $B$ &   2452761.81274 &         0.98689 &         0.00236 \\
     MagIC & $B$ &   2452761.81487 &         0.98643 &         0.00241 \\
     MagIC & $B$ &   2452761.81736 &         0.98923 &         0.00245 \\
     MagIC & $B$ &   2452761.83923 &         0.99126 &         0.00232 \\
     MagIC & $B$ &   2452761.84135 &         0.99121 &         0.00234 \\
     MagIC & $B$ &   2452761.84341 &         0.98534 &         0.00241 \\
     MagIC & $B$ &   2452761.84544 &         0.98779 &         0.00249 \\
     MagIC & $B$ &   2452761.84731 &         0.98854 &         0.00247 \\
     MagIC & $B$ &   2452761.85524 &         0.99267 &         0.00249 \\
     MagIC & $B$ &   2452761.85783 &         0.99182 &         0.00249 \\
     MagIC & $B$ &   2452761.85975 &         0.99178 &         0.00213 \\
     MagIC & $B$ &   2452761.86204 &         0.99363 &         0.00249 \\
     MagIC & $B$ &   2452761.86421 &         0.99561 &         0.00247 \\
     MagIC & $B$ &   2452761.86603 &         0.99929 &         0.00249 \\
     MagIC & $B$ &   2452761.86808 &         0.99672 &         0.00250 \\
     MagIC & $B$ &   2452761.87027 &         1.00124 &         0.00249 \\
     MagIC & $B$ &   2452761.87251 &         0.99817 &         0.00250 \\
     MagIC & $B$ &   2452761.87469 &         0.99722 &         0.00249 \\
     MagIC & $B$ &   2452761.87686 &         1.00267 &         0.00250 \\
     MagIC & $B$ &   2452761.87904 &         0.99946 &         0.00249 \\
     MagIC & $B$ &   2452761.88123 &         1.00011 &         0.00249 \\
     MagIC & $B$ &   2452761.88340 &         1.00464 &         0.00250 \\
     MagIC & $B$ &   2452761.88558 &         0.99980 &         0.00250 \\
     MagIC & $B$ &   2452761.88787 &         0.99985 &         0.00232 \\
     MagIC & $B$ &   2452761.89005 &         1.00144 &         0.00249 \\
     MagIC & $B$ &   2452761.89238 &         1.00456 &         0.00250 \\
     MagIC & $B$ &   2452761.89456 &         1.00211 &         0.00241 \\
     MagIC & $B$ &   2452761.89679 &         1.00036 &         0.00245 \\
     MagIC & $B$ &   2452761.89912 &         0.99888 &         0.00247 \\
     MagIC & $B$ &   2452761.90130 &         1.00048 &         0.00249 \\
     MagIC & $B$ &   2452761.90347 &         0.99610 &         0.00245 \\
     MagIC & $B$ &   2452761.90565 &         0.99743 &         0.00247 \\
     MagIC & $B$ &   2452761.90783 &         1.00092 &         0.00241 \\
     MagIC & $B$ &   2452761.91000 &         0.99963 &         0.00249 \\
     MagIC & $B$ &   2452761.91218 &         0.99768 &         0.00247 \\
     MagIC & $B$ &   2452761.91610 &         0.99840 &         0.00210 \\
     MagIC & $B$ &   2452761.91831 &         0.99810 &         0.00178 \\
     MagIC & $B$ &   2452761.92054 &         1.00192 &         0.00195 \\
     MagIC & $B$ &   2452761.92271 &         0.99954 &         0.00180 \\
     MagIC & $B$ &   2452761.92493 &         0.99760 &         0.00258 \\
     MagIC & $B$ &   2452761.92712 &         0.99738 &         0.00256 \\
     MagIC & $B$ &   2452761.92976 &         1.00588 &         0.00258 \\

